Provocation: Who benefits from "inclusion" in Generative AI?

The demands for accurate and representative generative AI systems means there is an increased demand on participatory evaluation structures. While these participatory structures are paramount to to ensure non-dominant values, knowledge and material culture are also reflected in AI models and the media they generate, we argue that dominant structures of community participation in AI development and evaluation are not explicit enough about the benefits and harms that members of socially marginalized groups may experience as a result of their participation. Without explicit interrogation of these benefits by AI developers, as a community we may remain blind to the immensity of systemic change that is needed as well. To support this provocation, we present a speculative case study, developed from our own collective experiences as AI researchers. We use this speculative context to itemize the barriers that need to be overcome in order for the proposed benefits to marginalized communities to be realized, and harms mitigated.

==> sections/99-main_tex.tex <==
\section{Introduction-old}

%A growing body of scholarship has demonstrated that despite record-breaking performance improvements on established benchmarks, state-of-the-art generative AI models fail to accurately represent and result in quality-of-service harms to socially marginalized groups \citep{hall2024towards,seth2024dosadatasetsocialartifacts,magomere2024eatfeedingfoundationmodels,mack2024they}.
Socially marginalized groups experience representational harms caused by state-of-the-art generative AI systems \citep{hall2024towards,seth2024dosadatasetsocialartifacts,magomere2024eatfeedingfoundationmodels,mack2024they}.
For example, popular text-to-image models (\nari{WWD example and Avery Mack example}).
In acknowledgment of these harms and a desire to build more inclusive AI models, there has been a recent ``participatory turn'' 
\citep{delgado2023participatoryturnaidesign} to include marginalized groups in AI development and evaluation \citep{suresh2024participation,young2024scale}.
One common model of participation is to engage community members in AI evaluation exercises, such as red-teaming or providing ``ground-truth'' labels for generated content related to their identity (\emph{e.g.}, \citep{hall2024towards,seth2024dosadatasetsocialartifacts,magomere2024eatfeedingfoundationmodels,mack2024they}).
Researchers often approach communities with the promise that 
their participation is crucial for improving both the quality-of-service that \emph{they} will experience, as end-users of generative AI systems; and for improving their community's societal-level representation in the media writ large \citep{}.

%However, this model of participation fails to consider 
While the benefits of engaging socially marginalized groups to improve group representations are clear to AI developers, it is unclear if, and how, the promised benefits to participants can be realized. For example, 



\nari{I think it would be powerful if we are able to find a quote from one of these references that clearly illustrates the above argument -- but we don't want to call out any single 1 paper.}

\nari{TODO add more references and papers to the above}

%foundation models drastically under-perform 

\color{gray}

\begin{enumerate}
    \item Marginalized groups are at present harmed by gen AI (quality-of-service errors). Examples: WWD, depictions of people with disabilities, etc. There has been a participatory turn towards including these communities in AI development. This participation takes many different forms. A common model of participation is to engage community members in providing ``ground-truth'' labels for their data with the promise that their participation is crucial to improving the quality of service \textit{they} will experience as end-users of GenAI systems. 
    \item However, this model of participation fails to consider (1) \textit{if communities of evaluators will be able to reliably access and use GenAI systems} and (2)  relies on `trickle-down effects'' logic where benefits to marginalized groups are contingent on more dominant groups' experiencing improved quality of service when using GenAI systems. 
    \item The benefits of this type of participation are clear to AI developers / technology companies. But the promised benefits to participants are unclear. It is critical that researchers seeking to involve participants in evaluations of system outputs concretely define \textit{What are participants getting out of  engaging in the evaluation process? And what are these benefits contingent on?}  
    \item Participants may actually be harmed by this model of participating. They are harmed in the near term because they have to be exposed to offensive or upsetting content and bear this burden more than overrepresented communities (Siobhan’s “paradox”). But also they may be harmed in the long term — for example, by impersonation, devaluation of actual real content about these communities, etc. Increased visibility might not always be desired.
    \item \textbf{Key thesis/provocation:} Researchers should pursue participatory engagements with marginalized communities only if they can define the benefits **to communities** for participating, on a specific time scale.
    \item
    \item
\end{enumerate}
  

%\section{Background on participatory AI}
\textbf{From Delgado et al}
"However, it is critical to acknowledge that some participation may not be better than no participation, in situations where participation is extractive (and thus harms participants [65, 203]), tokenistic in ways that reify or amplify existing power structures within participating communities or between stakeholders and designers [54], or cases where “pseudo-participation” [164] may foreclose or co-opt more meaningful forms of participation [54, 115]"

"As a starting point for meaningful participation, we call for practitioners to direct their attention toward explicating (a) the mechanisms of particular AI systems and (b) the potentials of AI broadly construed. This can be operationalized on three levels. 

(1) When designing AI systems, practitioners should consider ways to explain how a given AI system work as part of humans’ interactions with such a system. Much of the effort branded as Explainable AI falls under this pursuit [e.g., 67, 111, 131]. 

(2)During activities for stakeholder participation, practitioners should foster localized understandings of what a particular AI system in question can do and how such a system works. 

(3)And more fundamentally, practitioners should create opportunities to foster broad understandings of what AI can do and how AI works prior to participation"

\color{black}
\section{Speculative Case Study: How do community members realize benefits from improved GenAI performance?}
To illustrate the problematic nature of proclaimed participant benefits in the evaluation of GenAI outputs, we present a speculative case study tracing the flow of benefits from the GenAI model back to community members. We simplify the actors involved by categorizing them into three groups: AI developers, social actors, and community members. AI developers are engineers who work at large technology companies and build the components of GenAI models (e.g,...). Social actors are the people and organizations who use the output of GenAI models to create image media for commercial or personal purposes (e.g., marketing agencies, textbook publishers, freelance artists). Community members are the people who have ground-truth knowledge about what their community should look like in images. 

Deepika, a member of the blind low-vision community, is an adult woman living in India. She has been vision impaired since birth. She was invited to participate in a large technology company's data enrichment initiative to collect and label images of people in India who are blind or vision impaired. Deepika was told that she would benefit from the study because it would improve the \textit{quality of service} for a popular commercially-available text-to-image model generated images that would more accurately depict Indian people who are blind. Let's carefully interrogate this claimed benefit by asking: \textit{What are the benefits Deepika was promised contingent upon?} 

\newpage
\begin{figure}[H]
\centering
\includegraphics[width=1.2\linewidth]{figures/contingency_graph.png}
\caption{Temporary hold.
}
\label{fig:contingency-graph}
\end{figure}
The main benefit Deepika was promised was \textit{improved service quality}. This means that the model would be able to create accurate images of people who are blind in India. To realize this improved service quality, Deepika would have to be able to access the model on her own. For many marginalized communities, the simple act of model access is complicated by issues such as lack of reliable Internet connectivity [cite] and inaccessible user interfaces [cite]. Deepika is unlikely to be able to realize the benefits of the model's improved performance if she cannot reliably access and navigate its interface on her own.

Some researchers argue that community members like Deepika will benefit indirectly from improved service quality because other social actors, like marketing firms and textbook publishers, will get exposed to more accurate images by using GenAI systems. The core argument here is that GenAI systems will shape \textit{societal representation} and thus precipitate change in societal attitudes towards marginalized communities. For example, a marketing firm may use the GenAI model to create images for an ad campaign that shows people who are blind in India which is then seen by millions of people. Some of these people who are exposed to the marketing campaign may work at organizations that build physical infrastructure in India and they may start to advocate for accessible design of buildings to accommodate folks like Deepika. Therefore the model can be said to have contributed to societal representation that changes material circumstances for community members. 

However, changing societal representation is a long-term and uncertain process. Researchers cannot guarantee that social actors will use their models, let alone that they will use the images in an appropriate manner that portrays community members in a dignified light. Researchers cannot guarantee that accurately generated image representations will change the minds of people in positions of power to make changes to the material circumstances of community members. If we are asking community members to participate in generated image evaluation, an activity that is potentially harmful both in the moment and downstream, we owe it to our participants to be specific about exactly \textit{how} they would benefit and what their benefits are contingent on. 

\section{Critically assessing participation in evaluation}
\section{Key considerations for researchers pursuing participatory evaluation}
\begin{enumerate}
    \item Researchers should be transparent about benefits and harms.
    \item Involve participants in harm assessment. Participant should know how the outputs of their participation should be used, and be able to have more control over the outputs of their participation. --> supply chain transparency; investigating potential for watermarking data so participants can trace their engagement
    \begin{enumerate}
        \item \siobhan{tracking data being used - track uses of the data being used. Xinnuo's work for example}
        \item \siobhan{blog post about irresponsible webscraping - tracking who is coming to the website to figure out the data}
        \item \siobhan{How can people track their data being used on my behalf - third party audits}
        \item \siobhan{how can we \textit{honestly} elicit ongoing and informed consent when we don't actually understand how the models will be used. (Bogdana linkedin post). Genetic research - frequent opt / in out. Who will be contributing to the dataset}
        \item \siobhan{current definitions of how models work, how data will be used are very murky...value of data changes as models \& uses change. Be upfront and clear about we can't give control meaningfully - more honesty about the limitations of these systems. }
        \item \samantha{coming to terms with the fact of how far behind we are with the promises made about these.}
        \item \samantha{Be honest we don't know how they will be used long term, but we know who might benefit and what they might look like. Exercise for the team as a pre-activity (responsible ML/AI) -- translate options and implications -- tracing out logic actually . \textbf{Benefits may only come later with significant societal change, may only come later. Contigencies for benefits}}
        \item \samantha{Maybe explore data leverage in the context of GenAI https://dl.acm.org/doi/10.1145/3442188.3445885}
        \item 
    \end{enumerate}
    \item More research into how to sustain other models of participation beyond data labeling/data donation is needed — for example, more complex licensing, data stewardship, or even model development /ownership for community members, who are often resource-constrained.
\end{enumerate}

\textbf{What counts as a concrete benefit when participating in generative AI? }
1. The model will get better (address stereotypes, have accurate portrayals)
    --> Representational fidelity, you will be represented correctly 
    --> Preservation of material cultural 
    --> how do they know a model is getting better?
        --> would they need to buy access back to the model to use it? 
        --> WHO gets to use the model? Probably large advertising/marketing firms who can buy a license to the model. Yes this could improve "societal level" representation but utilizes trickle down logics

2. Access to information is not enough. Just because the models get better, still need community capacity to integrate it, feed models back into ecosystems in which they are being used. Can't just try ``improve'' representation and leave it at that

3. Outputs: control over these. GDPR -> implications of accepting different cookies.

Supply chain idea - Important because of how models work. Anyone can download the weights of a trained model
Tracking life of data given how models are trained and the representations are embedded. 

\section{proposals}

Activity a research group can step through to understand what the benefits are, what are they contingent on and how can they use this in their practice and informed consent etc. 

Good examples of informed consent in clinical trials research: https://www.ncbi.nlm.nih.gov/pmc/articles/PMC3601699/ 

FDA overview of informed consent in clinical trials research: 
https://www.fda.gov/patients/clinical-trials-what-patients-need-know/informed-consent-clinical-trials
